On the Generalization Power of Overfitted Two-Layer Neural Tangent Kernel Models

In this paper, we study the generalization performance of min $\ell_2$-norm overfitting solutions for the neural tangent kernel (NTK) model of a two-layer neural network with ReLU activation that has no bias term. We show that, depending on the ground-truth function, the test error of overfitted NTK models exhibits characteristics that are different from the "double-descent" of other overparameterized linear models with simple Fourier or Gaussian features. Specifically, for a class of learnable functions, we provide a new upper bound of the generalization error that approaches a small limiting value, even when the number of neurons $p$ approaches infinity. This limiting value further decreases with the number of training samples $n$. For functions outside of this class, we provide a lower bound on the generalization error that does not diminish to zero even when $n$ and $p$ are both large.

==> expressiveness.tex <==
\section{Expressiveness of $\hatf$}
With given $\Vzero$, we have
\begin{align*}
    \hatf(\xsmall)=\sum_{j=1}^p \bm{1}_{\{\xsmall^T\Vzeroj>0\}}\xsmall^T\DV[j].
\end{align*}
Define a function $\bm{J}:\mathds{R}^d\mapsto\mathds{R}^d$. If this function satisfies $\bm{J}(\Vzeroj)=\frac{1}{p}\DV[j]$ for all $j\in\{1,2,\cdots, p\}$, we have
\begin{align}\label{eq.temp_100201}
    \hatfJ(\xsmall)=\frac{1}{p}\sum_{j=1}^p\bm{1}_{\{\xsmall^T\Vzeroj>0\}}\xsmall^T\bm{J}(\Vzeroj).
\end{align}
In other words, for any $\Vzero$ and $\DV$, we can always find at least one such $\bm{J}$ that satisfies $\bm{J}(\Vzeroj)=\frac{1}{p}\DV[j]$ for all $j\in\{1,2,\cdots, p\}$. For any $\bm{J}$, we can let $\DV[j]=p\bm{J}(\Vzeroj)$ for all $j\in\{1,2,\cdots, p\}$. Therefore, we only need to study the expressiveness of Eq.~\eqref{eq.temp_100201}.

Let $\lambda_0(\cdot)$ define the distribution of $\frac{\Vzeroj}{\|\Vzeroj\|_2}$. We define
\begin{align*}
    \hatfJi(\xsmall)=\int_{\sd}\bm{1}_{\{\xsmall^T\bm{z}>0\}}\xsmall^T\bm{J}(\bm{z})d\lambda_0(\bm{z}).
\end{align*}

\begin{lemma}
For any $\bm{x}\in\sd$, we have
\begin{align*}
    \prob\left\{\left(\hatfJi(\xsmall)-\hatfJ(\xsmall)\right)^2\geq \TODO\right\}\leq \TODO.
\end{align*}
\end{lemma}
\begin{proof}
Chebyshev's inequality. \TODO.
\end{proof}

\subsection{When d=2}
We have
\begin{align*}
    \hatfJi(\theta)&=\int_{\theta-\frac{\pi}{2}}^{\theta+\frac{\pi}{2}}K(\varphi)\cos (D(\varphi)-\theta)d\varphi\\
    &=\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}K(\varphi+\theta)\cos(D(\varphi+\theta)-\theta)d\varphi\text{ (replace $d\varphi$ by $d(\varphi-\theta)$)}\\
    &=\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}\cos\theta K(\varphi+\theta)\cos(D(\varphi+\theta))d\varphi+\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}\sin\theta K(\varphi+\theta)\sin(D(\varphi+\theta))d\varphi\\
    &=\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}\cos\theta K(\theta-\varphi)\cos(D(\theta-\varphi))d\varphi+\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}\sin\theta K(\theta-\varphi)\sin(D(\theta-\varphi))d\varphi\text{ (replace $d\varphi$ by $d(-\varphi)$)}\\
    &=\cos\theta\int_\pi^\pi \bm{1}_{\{|\varphi|<\frac{\pi}{2}\}} L(\theta-\varphi)d\varphi+\sin\theta\int_\pi^\pi \bm{1}_{\{|\varphi|<\frac{\pi}{2}\}} T(\theta-\varphi)d\varphi
\end{align*}
where
\begin{align*}
    K=\sqrt{L^2+T^2},\quad \cos D=\frac{L}{\sqrt{L^2+T^2}},\quad \sin D=\frac{T}{\sqrt{L^2+T^2}}.
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% the following is the old part which is useless now

\begin{comment}
\newpage
{\color{gray}
\input{expressiveness}
}

\newpage
{\color{gray}
\begin{definition}
Define any vector $\DVs$ such that
\begin{align*}
    &\DVs\in \argmin_{\bm{v}\in\mathds{R}^{dp}}\ \expectation_{\xsmall}\left(\hx\bm{v}-\f(\xsmall)\right)^2.
\end{align*}
Define $\fs(\xsmall)\defeq\hx\DVs$.
\end{definition}

\begin{definition}\label{def.learnable}
A ground-truth $\f(\cdot)$ is called (overfitted-GD) learnable if $\hx\Ht^T(\Ht\Ht^T)^{-1}\F$ uniformly converges to $\fGD(\xsmall)$ (as $n\to\infty$) and   $\expectation_{\xsmall}(\fGD(\xsmall)-\f(\xsmall))^2=0$. Notice that $p\to\infty$ is required when $n\to\infty$ because $p\geq n/d$.
\end{definition}

\begin{lemma}
If $\f(\cdot)$ is learnable, then
\begin{align*}
    \lim_{p\to\infty} \expectation_{\xsmall}\left(\fs(\xsmall)-\f(\xsmall)\right)^2=0.
\end{align*}
\end{lemma}
\begin{proof}
By Definition~\ref{def.learnable}, we have
\begin{align*}
    \lim_{p\to\infty}\expectation_{\xsmall}(\fGD(\xsmall)-\f(\xsmall))^2=0.
\end{align*}
Thus, we have
\begin{align*}
    \lim_{p\to\infty}\min_{\bm{v}\in\mathds{R}^{dp}}\ \expectation_{\xsmall}\left(\hx\bm{v}-\f(\bm{x})\right)^2\leq \lim_{p\to\infty}\expectation_{\xsmall}(\hx\Ht^T(\Ht\Ht^T)^{-1}\F-\f(\xsmall))^2=0.
\end{align*}
Thus, we have
\begin{align*}
    \lim_{p\to\infty} \expectation_{\xsmall}\left(\fs(\xsmall)-\f(\xsmall)\right)^2=0.
\end{align*}
\end{proof}

\begin{proposition}
If $\fs(\cdot)$ is learnable, then $\f(\cdot)$ is learnable. If $\f(\cdot)$ is learnable, then $\fs(\cdot)$ is learnable.
\end{proposition}

By this proposition, to investigate which function is learnable, we can regard $\fs(\cdot)$ as ground-truth. 

\subsubsection{Bias term}
For min-$\ell_2$ solution of classical linear regression, when overfitting ($p>n$) happens, the bias term is non-zero (i.e., proportional to null risk). However, it does not happen here for, e.g., linear or constant ground truth. An intuitive explanation is that $\PH$ is an orthogonal projection to the row space of $\Ht$. As long as $\DVs$ is in/close to the row space of $\Ht$, then $(\PH-\identity)\DVs$ will be zero/small. Specifically, we have the following lemma.



\begin{enumerate}
    \item If the ground truth is constant, i.e., $f(\bm{x})=C$, then let $\bm{a}=\frac{2}{p}\cdot\frac{C\sqrt{2\pi d}}{n}[1\ 1\ \cdots\ 1]^T$.
    
    \item If the ground truth is linear, i.e., $f(\bm{x})=\bm{x}^T\bm{\beta}$, then let 
    \begin{align*}
        \bm{a}_i=\frac{2}{p}\cdot\frac{\sqrt{2\pi d}}{n}\text{sign}(\mathbf{X}_i^T\bm{\beta}).
    \end{align*}
\end{enumerate}



\subsubsection{Variance term}

\begin{align*}
    \|\hsmall\Ht^T\|_2\approx \sqrt{\frac{np}{2d}}
\end{align*}

\begin{align*}
    \|(\Ht\Ht^T)^{-1}\|_2=\frac{1}{\|\Ht\Ht^T\|_2}\approx \frac{1}{\sqrt{c_1\frac{np}{2}-c_2\frac{np}{d}}}\stackrel{\text{large } d}{\approx}\frac{c_3}{\sqrt{np}}
\end{align*}

\begin{align*}
    \|\hsmall\Ht^T(\Ht\Ht^T)^{-1}\epsilon\|_2\leq \sqrt{\frac{np}{2d}}\cdot \frac{c_3}{\sqrt{np}} \|\bm{\epsilon}\|_2=\frac{c_4}{d}\|\bm{\epsilon}\|_2.
\end{align*}
Notice that $c_1,c_2,c_3,c_4$ are related to the correlation between two $\mathbf{X}_j$ (or, $n$), when correlation is larger ($n$ is large), $c_1$ is smaller, $c_2$ is larger, then $c_3$ and $c_4$ are larger.

{function $f^*(\bm{x})$ that can be learnt with zero bias when $p\mapsto \infty$}

We use $f^*(\cdot)$ to denote such a function that can be learnt with zero bias. In this subsection, we only consider the situation of very large $p$, i.e., ignoring the randomness caused by finite $p$.


\begin{lemma}
For any $c\in \mathds{R}$, we have $f^*(c\bm{x})=cf^*(\bm{x})$ almost surely.
\end{lemma}

With this lemma, we can assume that all training and testing inputs are normalized, i.e., $\|\bm{x}\|_2=1$ and $\|\mathbf{X}_i\|_2=1$ for all $i\in\{1,\cdots,n\}$.

Let $\mu(\cdot)$ denote the probability density of input $\bm{x}$.

When $n$ is large, we have
\begin{align*}
    f^*(\bm{x})=\int_{\mathcal{S}^{d-1}}\frac{\pi-\arccos (\bm{x}^T\bm{z})}{\pi}(\bm{x}^T\bm{z}) g(\bm{z})d\mu(\bm{z})
\end{align*}




}
\end{comment}

==> proof_backward.tex <==
% \section{Proof of Theorem~\ref{th.backward}}\label{app.proof_backward}
\begin{proof}
% In order to show $\flinfSet=\learnableSet$, it only remains to prove $\flinfSet\subseteq \learnableSet$. To that end, l

Recall $\DX$ in Eq.~\eqref{eq.def_DX}. Define an event $\mathcal{J}$ as
\begin{align*}
    \mathcal{J}\defeq \left\{|\gbi|\leq \frac{n\|\ysmall\|_2}{\DX}\text{ for all }i=1,2,\cdots,n\right\}.
\end{align*}
We have
\begin{align}\label{eq.temp_020303}
    \prob_{\Vzero}\Big\{\frac{\min\eig\left(\Ht\Ht^T\right)}{p}\geq \DX\Big\}\geq 1-4ne^{-np\DX/6}\text{ (by Lemma~\ref{le.Ha_V0} and Lemma~\ref{le.min_eig})}.
\end{align}
By Lemma~\ref{le.matrix_norm}, we have
\begin{align}\label{eq.temp_020304}
    \gbi= np\bm{e}_i^T(\Ht\Ht^T)^{-1}\ysmall\leq \frac{np\|\ysmall\|_2}{\min\eig\left(\Ht\Ht^T\right)}.
\end{align}
By Eq.~\eqref{eq.temp_020303} and Eq.~\eqref{eq.temp_020304}, we have
\begin{align*}
    \prob_{\Vzero}\left\{|\gbi|\leq \frac{n\|\ysmall\|_2}{\DX}\ \bigg|\ i\right\}\geq 1-4ne^{-np\DX/6}.
\end{align*}
By the union bound, we thus have
\begin{align*}
    \prob_{\Vzero}\mathcal{J}\geq 1-4n^2e^{-np\DX/6}.
\end{align*}
By taking limits on both sides, we thus have
\begin{align}\label{eq.temp_020305}
    \lim_{p\to\infty}\prob_{\Vzero}\mathcal{J}=1.
\end{align}

Define
\begin{align*}
    f_{p}(\xsmall)\defeq \int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi d\xdensity(\bm{z}).
\end{align*}

When $\mathcal{J}$ happens, we have
\begin{align*}
    |f_p(\xsmall)| \leq \max_i |\gbi|\leq \frac{n\|\ysmall\|_2}{\DX}
\end{align*}

% By Lemma~\ref{le.lower_eig}, we know that for fixed $n$, when $p\to\infty$, $\gbi$ is upper-bounded by a value which is irrelevant to $p$ for all $i\in\{1,2,\cdots,n\}$ almost surely (randomness is based on $\XX$ and $\Vzero$). Therefore, we can find $U_n>0$ such that $|\gbi|\leq U_n$ holds for all $i\in\{1,2,\cdots,n\}$ and for any $p$ almost surely (randomness is based on $\XX$ and $\Vzero$). Thus,
% \begin{align}
%     \left\|\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}\gbi\right\|_1=\int_{\sd}\left|\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z})\gbi\right| d\xdensity(\bm{z})=\frac{1}{n}\sum_{i=1}^n|\gbi|\leq U_n<\infty,
% \end{align}
% which implies that $f_p\in \learnableSet$ for all $p$ almost surely. We can also show that (almost surely) for all $p$,
If $\mathcal{J}$ happens, then
\begin{align}\label{eq.temp_011709}
    \left\|\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}\gbi\right\|_1=\int_{\sd}\left|\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z})\gbi\right| d\xdensity(\bm{z})=\frac{1}{n}\sum_{i=1}^n|\gbi|\leq \frac{n\|\ysmall\|_2}{\DX},
\end{align}
which implies $f_p\in\learnableSet$ by Definition~\ref{def.learnableSet}.
We also have
\begin{align}
    \|\fl\|_2^2=&\int_{\sd}\left(\frac{1}{n}\sum_{i=1}^n\xsmall^T\Xii\frac{|\CXix|}{p}\gbi\right)^2 d\xdensity(\xsmall)\text{ (by Eq.~\eqref{eq.temp_012401})}\nonumber\\
    \leq &\int_{\sd}\left(\frac{1}{n}\sum_{i=1}^n|\gbi|\right)^2 d\xdensity(\xsmall)\text{ (because $|\xsmall^T\Xii|\leq 1$ and $\frac{|\CXix|}{p}\leq 1$)}\nonumber\\
    \leq &\left(\frac{n\|\ysmall\|_2}{\DX}\right)^2.\label{eq.temp_012402}
\end{align}


For all $\xsmall\in\sd$, we have
\begin{align*}
    \fl(\xsmall)-f_p(\xsmall)=\int_{\sd}\xsmall^T\bm{z}\left(\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right)\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi d\xdensity(\bm{z}).
\end{align*}
Because $|\xsmall^T\bm{z}|\leq 1$, $\frac{|\Czx|}{p}\leq 1$, and $\left|\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right|\leq \frac{1}{2}$, we have
\begin{align}\label{eq.temp_101801}
    |\fl(\xsmall)-f_p(\xsmall)|\leq& \int_{\sd}|\xsmall^T\bm{z}|\cdot\left|\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right|\cdot\left|\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi\right| d\xdensity(\bm{z})\nonumber\\
    \leq & \frac{3n\|\ysmall\|_2}{2\DX}\text{ (by Eq.~\eqref{eq.temp_011709})},
\end{align}

Define the event $\mathcal{K}$ that
\begin{align*}
    \mathcal{K}\defeq\left\{\left|\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right|\leq \zeta\right\}.
\end{align*}
By Lemma~\ref{le.c_divide_p_convergence}, there exists a threshold $p_0$ such that for all $p>p_0$, for all $\xsmall\in\sd$, $\prob_{\Vzero}[\mathcal{K}]\geq 1-\zeta$.

By Eq.~\eqref{eq.temp_020305}, there exist a threshold $p_1$ such that for all $p>p_1$, $\prob_{\Vzero}[\mathcal{J}]\geq 1-\zeta$.

If $\mathcal{J}$ and $\mathcal{K}$ happens, then we have
\begin{align*}
    |\flmap(\xsmall)-f_p(\xsmall)|=&\left|\int_{\sd}\xsmall^T\bm{z}\left(\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right)\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi d\xdensity(\bm{z})\right|\\
    \leq & \int_{\sd}|\xsmall^T\bm{z}|\left|\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right|\cdot \left|\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi\right| d\xdensity(\bm{z})\\
    \leq &\zeta \frac{n\|\ysmall\|_2}{\DX}.
\end{align*}

Thus, for all $p>\max\{p_0,p_1\}$, for all $\xsmall\in\sd$, we have
\begin{align*}
    \prob_{\Vzero}\left\{|\fl(\xsmall)-f_p(\xsmall)|\leq \zeta \frac{n\|\ysmall\|_2}{\DX}\right\}\geq 1-2\zeta \text{ (by the union bound)}.
\end{align*}
Thus, we have
\begin{align*}
    \prob_{\Vzero,\xsmall}\left\{|\fl(\xsmall)-f_p(\xsmall)|\leq \zeta \frac{n\|\ysmall\|_2}{\DX}\right\}\geq 1-2\zeta.
\end{align*}

Define
\begin{align*}
    M\defeq(\text{bound of }\f) +  \frac{n\|\ysmall\|_2}{\DX}.
\end{align*}

Because
\begin{align*}
    \int_{\sd}(\f(\xsmall)-f_p(\xsmall))^2 d\xdensity(\xsmall)=\|\f-f_p\|_2^2\geq (D(\f,\learnableSet))^2,
\end{align*}
we have
\begin{align*}
    \prob_{\xsmall,\Vzero}\left\{(\f(\xsmall)-f_p(\xsmall))^2\geq \frac{(D(\f,\learnableSet))^2}{2}  \big|\  \mathcal{J}\right\}\geq\frac{(D(\f,\learnableSet))^2}{2M}.
\end{align*}
Thus,
\begin{align*}
    \prob_{\xsmall,\Vzero}\left\{|\f(\xsmall)-f_p(\xsmall)|\geq \frac{D(\f,\learnableSet)}{\sqrt{2}}\right\}\geq\prob_{\xsmall,\Vzero}\left\{|\f(\xsmall)-f_p(\xsmall)|\geq \frac{D(\f,\learnableSet)}{\sqrt{2}}, \mathcal{J}\right\}\geq\frac{(D(\f,\learnableSet))^2}{2M}(1-\zeta).
\end{align*}

Thus, we have
\begin{align*}
    &\prob_{\xsmall,\Vzero}\left\{|f(\xsmall)-\fl(\xsmall)|\geq \frac{D(\f,\learnableSet)}{\sqrt{2}} - \zeta \frac{n\|\ysmall\|_2}{\DX} \right\}\\
    \geq & 1 - \prob_{\xsmall,\Vzero}\left\{|\fl(\xsmall)-f_p(\xsmall)|\leq \zeta \frac{n\|\ysmall\|_2}{\DX}\right\} - \prob_{\xsmall,\Vzero}\left\{|\f(\xsmall)-f_p(\xsmall)|\leq \frac{D(\f,\learnableSet)}{\sqrt{2}} \right\}\\
    \geq & 1- 2\zeta - \left(1-\frac{(D(\f,\learnableSet))^2}{2M}(1-\zeta)\right)\\
    =&\frac{(D(\f,\learnableSet))^2}{2M}(1-\zeta)-2\zeta.
\end{align*}


% If $J$ happens, then for any $\xsmall\in\sd$, we have
% \begin{align*}
%     &\lim_{p\to\infty}|\flmap(\xsmall)-f_p(\xsmall)|\\
%     =&\lim_{p\to\infty}\left|\int_{\sd}\xsmall^T\bm{z}\left(\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right)\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi d\xdensity(\bm{z})\right|\\
%     =&\left|\int_{\sd}\xsmall^T\bm{z}\lim_{p\to\infty}\left(\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right)\frac{1}{n}\sum_{i=1}^n\delta_{\Xii}(\bm{z}) \gbi d\xdensity(\bm{z})\right|\\
%     &\text{ (by bounded convergence theorem and Eq.~\eqref{eq.temp_101801})}.
% \end{align*}
% By Lemma~\ref{le.spherePortion}, we know that
% \begin{align*}
%     \left(\frac{|\Czx|}{p}-\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}\right)\stackrel{\text{P}}{\rightarrow}0.
% \end{align*}
% Thus, if $J$ happens, then
% \begin{align*}
%     |\flmap(\xsmall)-f_p(\xsmall)|\stackrel{\text{P}}{\rightarrow}0.
% \end{align*}
% By Eq.~\eqref{eq.temp_020305}, we know that $J$ is very likely to happen when $p$ is sufficiently large (i.e., converges in probability as $p\to\infty$). The result of this lemma thus follows.
\end{proof}


\begin{comment}
When $d=2$, the 2-D vector $\Xii$ can be replaced by its angle $\theta_i$ on the 2-D plane. Thus, we have
\begin{align*}
    \flinf(\varphi)=\int_{\varphi-\pi}^{\varphi+\pi}\frac{\pi-|\theta-\varphi|}{\pi}\cos(\theta - \varphi)\frac{1}{n}\sum_{i=1}^n\delta_{\theta_i}(\theta)\gbinf d\theta.
\end{align*}
Compared with the functions in $\learnableSet$, the only difference is that $\frac{1}{n}\sum_{i=1}^n\delta_{\theta_i}(\bm{z})\gbinf$ may be not in $L^2$ (because Dirac delta function has infinite $L^2$ norm). Nonetheless, we can still do orthogonal decomposition of $\frac{1}{n}\sum_{i=1}^n\delta_{\theta_i}(\bm{z})\gbinf$. Specifically, we have
\begin{align*}
    \frac{1}{n}\sum_{j=1}^n\delta_{\theta_j}(\bm{z})\gbinfj=\sum_{k=-\infty}^\infty \left(\frac{1}{2n\pi}\sum_{j=1}^n e^{-ik\theta_j}\gbinfj \right)e^{ik\varphi}.
\end{align*}
Thus, similar to what we did in the proof of Proposition~\ref{prop.d2}, the conclusion of this proposition thus follows.

% we have
% \begin{align*}
%     \sum_{k=2,4,\cdots}\frac{a_k^2+b_k^2}{\left(\frac{1}{(k+1)^2}+\frac{1}{(k-1)^2}\right)^2}=\sum_{k=\pm 2,\pm 4,\cdots}\left|\frac{1}{2n\pi}\sum_{j=1}^n e^{-ik\theta_j}\gbinfj\right|^2.
% \end{align*}
\end{comment}







==> proof_linear.tex <==
\section{Linear functions}\label{app.proof_linear}
It is obvious that $\learnableSet$ contains some non-linear functions by Definition~\ref{def.learnableSet}. In contrast, it is not so obvious on whether $\learnableSet$ contains linear functions. Indeed, we prove that $\learnableSet$ does contain all linear functions, which is formally stated in Proposition~\ref{prop.linear} as follows.
\begin{proposition}\label{prop.linear}
$\learnableSet$ includes linear functions. Specifically, define the set of all linear functions as
\begin{align*}
    \learnableSet\supseteq\linearSet\defeq\left\{\f:\ \sd\mapsto\mathds{R}\ \big|\ \f(\xsmall)=\xsmall^T\bm{a}+b,\ \bm{a}\in \mathds{R}^d,\ b\in\mathds{R}\right\}.
\end{align*}
\end{proposition}

\begin{proof}
To show $\linearSet\subseteq \learnableSet$, we need to construct a $L^2$ function $g$ such that $\fg=\xsmall^T\bm{a}+b$. To this end, we construct $g$ as
\begin{align*}
    g(\bm{z})=\begin{cases}
    C+D,\quad&\text{ if }\bm{z}^T\bm{a}>0,\\
    -C+D,&\text{ otherwise},
    \end{cases}
\end{align*}
where
\begin{align*}
    &C=\|\bm{a}\|_2\left(\int_{\sd}\bm{1}_{\{\xsmall^T\bm{v}>0\}}\int_{\sd}\bm{z}^T\bm{e} \bm{1}_{\{\bm{z}^T\bm{e}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})\right)^{-1},\\
    &D=b\left(\int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi} d\xdensity(\bm{z})\right)^{-1}.
\end{align*}
It remains to check that $\fg=\xsmall^T\bm{a}+b$. Case 1: $\bm{a}=0$. In this case, we have
\begin{align*}
    \fg(\xsmall)&=\int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}D d\xdensity(\bm{z})\\
    &=D\int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi} d\xdensity(\bm{z})\\
    &=b\text{ (by plugging the value of $D$)}\\
    &=\bm{x}^T\bm{a}+b\text{ (because $\bm{a}=0$)}.
\end{align*}
Case 2: $\bm{a}\neq \bm{0}$. We have
\begin{align*}
    \fg(\xsmall)=&\int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}(g(\bm{z})-D) d\xdensity(\bm{z})+\int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}D d\xdensity(\bm{z})\\
    =&\int_{\sd}\xsmall^T\bm{z}\frac{\pi-\arccos (\xsmall^T\bm{z})}{2\pi}(g(\bm{z})-D) d\xdensity(\bm{z})+b\text{ (proved in Case 1)}\\
    =&\int_{\sd}\int_{\sd}\xsmall^T\bm{z} \bm{1}_{\{\bm{z}^T\bm{v}>0,\ \xsmall^T\bm{v}>0\}}g(\bm{z}) d\xdensity(\bm{z})d\nvdensity(\bm{v})+b\text{ (by Lemma~\ref{le.change_seq})}\\
    =&C\int_{\sd}\int_{\sd}\xsmall^T\bm{z} \bm{1}_{\{\bm{z}^T\bm{v}>0,\ \xsmall^T\bm{v}>0,\ \bm{z}^T\bm{a}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})\\
    &-C\int_{\sd}\int_{\sd}\xsmall^T\bm{z} \bm{1}_{\{\bm{z}^T\bm{v}>0,\ \xsmall^T\bm{v}>0,\ \bm{z}^T\bm{a}<0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})+b\\
    =&C\int_{\sd}\int_{\sd}\xsmall^T\bm{z} \bm{1}_{\{\bm{z}^T\bm{v}>0,\ \xsmall^T\bm{v}>0,\ \bm{z}^T\bm{a}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})\\
    &+C\int_{\sd}\int_{\sd}\xsmall^T\bm{z} \bm{1}_{\{\bm{z}^T\bm{v}<0,\ \xsmall^T\bm{v}>0,\ \bm{z}^T\bm{a}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})+b\\
    &\text{ (replace $\bm{z}$ by $-\bm{z}$ in the second term)}\\
    =&C\int_{\sd}\int_{\sd}\xsmall^T\bm{z} \bm{1}_{\{\xsmall^T\bm{v}>0,\ \bm{z}^T\bm{a}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})+b\\
    =&C\xsmall^T\int_{\sd}\int_{\sd}\bm{z} \bm{1}_{\{\xsmall^T\bm{v}>0,\ \bm{z}^T\bm{a}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})\\
    =&C\xsmall^T\int_{\sd}\bm{1}_{\{\xsmall^T\bm{v}>0\}}\int_{\sd}\bm{z} \bm{1}_{\{\bm{z}^T\bm{a}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})+b\\
    =&\xsmall^T\bm{a}\left(\frac{C}{\|\bm{a}\|_2}\int_{\sd}\bm{1}_{\{\xsmall^T\bm{v}>0\}}\int_{\sd}\bm{z}^T\bm{e} \bm{1}_{\{\bm{z}^T\bm{e}>0\}} d\xdensity(\bm{z})d\nvdensity(\bm{v})\right)+b\text{ (by Lemma~\ref{le.symmetry})}\\
    =&\xsmall^T\bm{a}+b\text{ (by plugging the value of C)}.
\end{align*}
In conclusion, for both cases, we have $\fg=\bm{x}^T\bm{a}+b$. The result of Proposition~\ref{prop.linear} thus follows.
\end{proof}

==> proof_lower_bound_error.tex <==
% \section{Proof of Proposition~\ref{prop.lower_bound_error}}\label{app.proof_lower_bound_error}

% Now we are ready to prove Proposition~\ref{prop.lower_bound_error}. 


==> sketch_proof_no_noise.tex <==
% \section{Sketched proof of Proposition~\ref{th.large_p}}
Here we briefly explain the idea of the proof of Proposition~\ref{th.large_p}. To estimate $|\fl(\xsmall)-\f(\xsmall)|$ when both $\Vzero$ and $\XX$ are random, we adopt the corresponding pseudo ground-truth as a ``middleware''. We define the output of the pseudo ground-truth for training input as $\Fv(\XX)\defeq[\fv(\XX_1)\ \fv(\XX_2)\ \cdots\ \fv(\XX_n)]^T$. We then split $\fl(\xsmall)-\f(\xsmall)$ by three terms.
\begin{align*}
    &\underbrace{\left(\hx\Ht^T(\Ht\Ht^T)^{-1}\Fv(\XX)-\fv(\xsmall)\right)}_{\text{term }A}+\underbrace{\left(\hx\Ht^T(\Ht\Ht^T)^{-1}\left(\F(\XX)-\Fv(\XX)\right)\right)}_{\text{term }B}\nonumber\\
    &+\underbrace{\left(\fv(\xsmall)-\f(\xsmall)\right)}_{\text{term }C}.
\end{align*}
The term $A$ corresponds to the test error of pseudo ground-truth, the term $B$ corresponds to the impact of the difference between pseudo ground-truth and real ground-truth in the training data, and the term $C$ corresponds to the impact of the difference between pseudo ground-truth and real ground-truth in the test data. In the sense of bias-variance decomposition, term $A$ is the ``pseudo bias'' and term $B$ is the ``pseudo variance''. 

Term $A$ has been bounded by Proposition~\ref{th.fixed_Vzero}. Because of Lemma~\ref{le.spherePortion}, as $p\to \infty$, we know pseudo ground-truth approaches the ground-truth, i.e., both $\fv(\xsmall)-\f(\xsmall)$ and $\F(\XX)-\Fv(\XX)$ approach $0$. Thus, term $B$ and term $C$ approach $0$ when $p\to \infty$. The convergence speed can be estimated by the Chernoff bound. Notice that we also need to use the conclusion of Proposition~\ref{prop.noise_large_p} to bound term $B$ (as term $B$ represents the ``pseudo variance''). The conclusion of Proposition~\ref{th.large_p} follows by combining the results of estimating terms $A$, $B$, and $C$.

==> tri_integral.tex <==
\begin{lemma}
When $a^2\neq b^2$ and $C$ is a constant, we have
\begin{align*}
    &\int (\sin ax)(\cos bx)\,dx=-{\frac {\cos((a-b)x)}{2(a-b)}}-{\frac {\cos((a+b)x)}{2(a+b)}}+C,\\
    &\int x \sin(a x) \cos(b x) dx = \frac{1}{2} \left(\frac{\sin(x (a - b))}{(a - b)^2} + \frac{\sin(x (a + b))}{(a + b)^2} - \frac{x \cos(x (a - b))}{a - b} - \frac{x \cos(x (a + b))}{a + b}\right) + C,\\
    &\int \cos(x) \sin(x) dx = -\frac{1}{2} \cos^2(x) + C,\\
    &\int  x \cos(x) \sin(x) dx = \frac{1}{8} (\sin(2 x) - 2 x \cos(2 x)) + C.
\end{align*}
\end{lemma}
\begin{proof}
\TODO
\end{proof}
